Furstenberg sets in finite fields: Explaining and improving the Ellenberg-Erman proof

A $(k,m)$-Furstenberg set is a subset $S \subset \mathbb{F}_q^n$ with the property that each $k$-dimensional subspace of $\mathbb{F}_q^n$ can be translated so that it intersects $S$ in at least $m$ points. Ellenberg and Erman proved that $(k,m)$-Furstenberg sets must have size at least $C_{n,k}m^{n/k}$, where $C_{n,k}$ is a constant depending only $n$ and $k$. In this paper, we adopt the same proof strategy as Ellenberg and Erman, but use more elementary techniques than their scheme-theoretic method. By modifying certain parts of the argument, we obtain an improved bound on $C_{n,k}$, and our improved bound is nearly optimal for an algebraic generalization the main combinatorial result. We also extend our analysis to give lower bounds for sets that have large intersection with shifts of a specific family of higher-degree co-dimension $n-k$ varieties, instead of just co-dimension $n-k$ subspaces.

==> betterBounds.tex <==
\section{A more nuanced bound for Furstenberg Algebras}\label{sec:nuancedBound}
% For a $(k,m)$-Furstenberg set with $m=(o(q))^k$ we can produce better bounds. We do this by proving the following theorem.
Using the tools developed so far, we are going to produce better bound for certain values of $m,q$ and $n$ for Furstenberg Sets. The first step is to produce a more nuanced bound for $(n-1,m)$-Hom-Furstenberg Algebras for large enough $m$ which will be used to prove Theorem \ref{parametricBound}

\begin{thm}\label{explicitHomFrust}
Given an $(n-1,m)$-Hom-Furstenberg Algebra $R=\F_q[x_1,\hdots,x_n]/I$ we have for all $m\ge (e^2n)^n$,
$$\text{dim}_{\F_q} R\ge F(n,m,q)m^{n/(n-1)},$$
where 
$$ F(n,m,q)=\left(e\left(1+\frac{m^{1/(n-1)}}{eq}\right)^{1/(n-1)}+\frac{m^{1/(n-1)}}{q}\right)^{-1}.$$
\end{thm}
\begin{proof}
Given an $(n-1,m)$-Furstenberg Algebra $R$ we consider the ideal $J_l(R)$ for integer $l$. 
% If $J_m(R)=0$ then using Theorem \ref{thm:furstPlaneZero} we have the bound
% $$|R| \ge D(n,m)m^{n/(n-1)},$$
% which suffices for our purposes. If $J_m(R)\ne 0$ 
We find the smallest $l$ such that $J_l(R)=\langle 0\rangle $. This exists because $J_0(R)=\langle 0\rangle $ as all hyperplanes will $(R,0)$-rich. Now using Theorem \ref{thm:furstPlaneZero} we have,
\begin{align}
    \text{dim}_{\F_q} R \ge \left(\frac{l}{m}\right)^{n/(n-1)}D(n,l)m^{n/(n-1)}.\label{boundk1}
\end{align}
For a fixed $n$, we can replace $D(n,l)$ with $d_n(l)$. We also have that $J_{l+1}(R)\ne \langle 0\rangle$. Using Theorem \ref{thm:furstPlaneNon} we have,
\begin{align}
    \text{dim}_{\F_q} R \ge qm\left(1-\frac{l}{m}\right).\label{boundk2}
\end{align}
Combining \eqref{boundk1} and \eqref{boundk2} together we get,
\begin{align}
\text{dim}_{\F_q} R \ge \max\left(\left(\frac{l}{m}\right)^{n/(n-1)}d_n(l)m^{n/(n-1)},qm\left(1-\frac{l}{m}\right)\right).\label{boundk3} 
\end{align}
%  We note \eqref{boundk1} increases as $k$ does while \eqref{boundk2} is decreasing in $k$. This means to minimize \eqref{boundk3} we need to find a $k$ for which the two terms match. Let $k/m=f$.
To find a general bound we need to find the minimum of \eqref{boundk3} as we vary $l$ over non-negative integers. Using Theorem \ref{thm:furstPlaneZero}, we note \eqref{boundk1} increases as $l$ varies over the non-negative {\bf reals}. Equation \eqref{boundk2} is decreasing in $l$ over the non-negative {\bf reals}. This means to simply find a universal lower bound we can just pick any real value for $l$ and take the minimum of the two expressions. We use,
\begin{align}
    l= m\frac{(1+f)^{1/(n-1)}}{((1+f)^{1/(n-1)}+f)}\label{eq:lvaluekbound}
\end{align}
where $f=m^{1/(n-1)}(qe)^{-1}$ and pick the smaller expression. First, we analyse $d_n(l)$. To that end, we make the following claim,
\begin{claim}
As $m\ge (e^2n)^n$, we have $l\ge (e^2n)^{n-1}$.
\end{claim}
\begin{proof}
We prove the statement in two cases. 

{\bf Case 1) $n=2$ or $f\le (1+f)^{1/(n-1)}$: }
\begin{align*}
l&=\frac{(1+f)^{1/(n-1)}m}{(1+f)^{1/(n-1)}+f} &\\
&\ge \frac{m}{2}\ge (e^2n)^{n-1}.
\end{align*}

{\bf Case 2) $n\ge 3$ and $f\ge (1+f)^{1/(n-1)}$: }
\begin{align*}
l&=\frac{(1+f)^{1/(n-1)}m}{(1+f)^{1/(n-1)}+f} &\\
&\ge \frac{f^{1/(n-1)}m}{2f} &\text{(As $f\ge (1+f)^{1/(n-1)}$ and $1+f\ge f$)}\\
&\ge m^{1-(n-2)/(n-1)^2}\frac{(qe)^{(n-2)/(n-1)}}{2} & \text{(substituting for $f$)}\\
&\ge m^{1-(n-2)/(n-1)^2} & \text{(As for $n\ge 3$, $(qe)^{(n-2)/(n-1)}\ge (2e)^{1/2}\ge 2$)}\\
&\ge m^{n/(n-1)} & \text{(As $1/n\ge (n-2)/(n-1)^2$)}\\
&\ge (e^2n)^{n-1}.
\end{align*}
\end{proof}

Using Theorem \ref{thm:furstPlaneZero} and the claim above we have $d_n(l)\ge e^{-1}$. Now we are ready to prove a general bound by substituting \eqref{eq:lvaluekbound} in \eqref{boundk2} and \eqref{boundk1}, and taking their minimum.
\begin{align*}
    \text{dim}_{\F_q} R &\ge \min\left(\frac{(1+f)^{n/(n-1)^2}}{((1+f)^{1/(n-1)}+f)^{n/(n-1)}}d_n(l)m^{n/(n-1)},m\frac{f}{(1+f)^{1/(n-1)}+f}\right) \\
     &\ge \frac{e^{-1}m^{n/(n-1)}}{((1+f)^{1/(n-1)}+f)}\min\left(\left(\frac{(1+f)^{n/(n-1)}}{(1+f)^{1/(n-1)}+f}\right)^{1/(n-1)},1\right)\\
    &\ge \frac{e^{-1}m^{n/(n-1)}}{((1+f)^{1/(n-1)}+f)}.
\end{align*}
Substituting $f=m^{1/(n-1)}(qe)^{-1}$ above gives the required bound.
% Setting $E(n,m)=D(n,k)$ we are done proving the bound. Using Theorem \ref{thm:furstPlaneZero}, we know $D(n,k)\ge 1/4$ which proves $E(n,m)\ge 1/4$. If $m\ge (e^2n)^n$ we have,
% $$k=\frac{(1+d)^{1/(n-1)}m}{(1+d)^{1/(n-1)}+d}\ge \frac{m}{d^{(n-2)/n-1}}\ge m^{1-(n-2)/(n-1)^2}\ge m^{(n-1)/n}\ge (e^2n)^{n-1}.$$
% Using Theorem \ref{thm:furstPlaneZero}, we have $E(n,m)=D(n,k)\ge 1/e$.
\end{proof}

% We note
% $$\prod\limits_{i=k+1}^{n}D(i,m)^{n/i}=\Big(\frac{k!^{n/k}}{n!}+o(1)\Big),$$
% where $o(1)$ is a term which goes to $0$ when $n$ is fixed and $q$ grows to infinity. We also have $D(n,m)\le 1$. Now given a $(k,m)$-Hom-Furstenberg Algebra and applying Lemma \ref{explicitHomFrust} and Lemma \ref{recurseBound} gives us,
% $$|R|\ge m^{n/k}\prod\limits_{i=k+1}^n\Big(\frac{D(i,m)}{(m^{1/k}D(i,m)q^{-1}+1-1/q)^{i/(i-1)}}\Big)^{n/i}.$$
% If we know $m=(o(q))^k$ then we have,
% $$|R| \ge m^{n/k}\prod\limits_{i=k+1}^n\Big(\frac{D(i,m)}{(o(q)D(i,m)q^{-1}+1-1/q)^{i/(i-1)}}\Big)^{n/i}\ge m^{n/k}\Big(\frac{k!^{n/k}}{n!}+o(1)\Big),$$
% where $o(1)$ is a term which goes to $0$ when $n$ is fixed and $q$ goes to $\infty$. In this special case we match the upper bounds on the constant in Theorem \ref{AlgebraBound} asymptotically in $q$. Lemma \ref{DFrustLem} lets us lift this bound to Furstenberg Algebras. Corollary \ref{FrustSet2Alg} lets us lift the Furstenberg Algebra bound to Furstenberg sets proving Theorem \ref{SetTheorem} when $m=(o(q))^k$ with $C_{n,k}=O(e^{n\log(n/k)})+o(1)$. For Kakeya sets we know the constant is $1/2^n$. For this reason we expect the bound for Furstenberg sets to be better than this. Ideally we expect the constant to be at least $C_{n,k}=2^{k-n}$ for all values of $m$.
% We will now randomly throw away points in other settings to extend this bound further.
\section{Algebras produced from polynomials with higher multiplicities}\label{sec:HigherMultAlgebra}
We need to generalize the construction $\text{Alg}(S)$ to take into account multiplicities of polynomials vanishing on it. We will analyse these algebras using Theorem \ref{explicitHomFrust} to prove Theorem \ref{parametricBound}.
\begin{define}[Algebras with multiplicity from Point sets]
Given a point set $S$ in $\F^n$ define the ideal $\I^{(l)}_\F(S)$ as the ideal of polynomials which vanish on $S$ with multiplicity at least $l$. 
We then define $\text{Alg}^{(l)}(S)$ to be the $\F$-algebra $\F[x_1,\hdots,x_n]/\I^{(l)}_\F(S)$.
\end{define}

Note, $\I^{(l)}_\F(S)$ is precisely the $l$th differential power of $\I_\F(S)$ which is the same as the $l$th symbolic power of $\I_\F(S)$ due to the Zariski-Nagata Theorem. We state these facts for awareness and will not be using them. More details can be found in \cite{eisenbud1995commutative}.

Again, in dimension $1$ the picture is simple. For example take the point set $S=\{0,1\}\subseteq \F$. We see any polynomial in $\F[x]$ which vanishes on $S$ with multiplicity $3$ belongs to the ideal $\langle x^3(x-1)^3\rangle$. Therefore, $\text{Alg}^{(3)}(S)=\F[x]/\langle x^3(x-1)^3\rangle$. Evaluating polynomials and all its Hasse derivatives of weight strictly less than $3$ at $0$ and $1$ produces an isomorphism of vector spaces from $\F[x]$ to $\F^{2\times 3}$. This shows $\text{Alg}^{(3)}(S)$ is of dimension $2\times 3$. Take a polynomial $f(x)$ such that $f(0)=0$ and $f(1)\ne 0$. Using the isomorphism induced by the evaluation map $\F[x]\rightarrow \F^{2\times 3}$ it is not hard to check that $\text{Alg}(S)/\langle f(x)\rangle$ is of dimension at least $3$ corresponding to the evaluation of polynomials and their Hasse derivatives on $1$. Fortunately, this picture holds true in general.

\begin{prop}[Geometry of higher multiplicity algebras]\label{point2algebraRedux}
Given a finite set $S$ of points in $\F^n$, the $\F$-algebra, $\text{Alg}^{(l)}(S)=\F[x_1,\hdots,x_n]/\I_\F^{(l)}(S)$ satisfies the following properties:
\begin{enumerate}
    \item $\text{Alg}^{(l)}(S)$ is a $\F$-vector space of dimension $|S|{l + n - 1 \choose n}$.

    \item A $k$-dimensional $(S,m)$-rich subspace $W$, is $(\text{Alg}^{(l)}(S), m')$-rich where $m'\ge m{l + k - 1 \choose k}$.
\end{enumerate}
\end{prop}
\begin{proof}
Let ${l + n - 1 \choose n}=L$. For every point $b\in S$ we can define the map $\text{Eval}_{b,l}:\F[x_1,\hdots,x_n]\rightarrow \F^{L}$ which simply evaluates a polynomial and all its Hasse derivatives of weight strictly less than $l$ at the point $b$. This map is the same as the canonical quotient map $\F[X]\rightarrow \F[X]/\langle X-b\rangle^l$ where $X=(x_1,\hdots,x_n)$ and $\langle X-b\rangle=\langle x_1-b_1,\hdots,x_n-b_n\rangle$. This means the map is a ring homomorphism and in particular is linear in $\F$. 

Combining the $|S|$ evaluation maps together for each point in $b$ we have the map $\text{Eval}_{S,l}:\F[x_1,\hdots,x_n]\rightarrow R=\bigoplus_{b\in S}\F[X]/\langle X-b\rangle^l \cong \F^{|S|L}$. The kernel of this map is precisely going to be $\I_\F^{(l)}(S)$ the ideal of polynomials vanishing on $S$ with multiplicity $l$. This means $\text{Eval}_{S,l}$ factors via an injective map $\phi$ from $\text{Alg}^{(l)}(S)=\F[x_1,\hdots,x_n]/\I_\F^{(l)}(S)$ to $R\cong \F^{|S|L}$ and the quotient map $\F[x_1,\hdots,x_n]\rightarrow \text{Alg}^{(l)}(S)$. By construction $\phi$ maps any element of $\text{Alg}^{(l)}(S)$ to its evaluation and its Hasse derivatives of weight at most $l$ over $S$. This proves that $\text{Alg}^{(l)}(S)$ is finite dimensional.

\begin{center}\begin{tikzcd}
\F[x_1,\hdots,x_n]\arrow[rd]\arrow[r, "\text{Eval}_{S,l}"] & R=\bigoplus_{b\in S} \F[X]/\langle X-b\rangle^l \cong \F^{|S|L} \\
& \text{Alg}^{(l)}(S) \arrow[u, "\phi"]
\end{tikzcd}\end{center}

% Coordinate wise addition and multiplication bestows on $\F^{|S|}$ a ring structure with $(1,1,\hdots,1)$ as the unit and the origin as the zero. Indeed, it is an easy check that $\text{Eval}_S$ is a ring map. 

Let $[N]=\{1,\hdots,N\}$ for any natural number $N$. For all points $b\in S$ we can find $f_b$ which vanish on $|S|\setminus\{b\}$ and not on $b$ using interpolation. $f_b^l$ vanishes on $|S|\setminus \{b\}$ with multiplicity at least $l$ and doesn't vanish on $b$. For some $b\in S,t\in \Z_{\ge 0},\text{wt}(t)<l$ consider the polynomial $f_{b,t}=f^l_b\prod_{i=1}^n (x_i-b_i)^{t_i}$. $f_{b,t}$ vanishes on $|S|\setminus \{b\}$ with multiplicity at least $l$. Using Lemma \ref{derivativeRule}, we also see all Hasse derivatives of $f_{b,t}$ of weight strictly less than $\text{wt}(t)$ vanish on $b$. Using Lemma \ref{derivativeRule}, we also note the only weight $\text{wt}(t)$ Hasse derivative of $f_{b,t}$ which does not vanish on $b$ is the Hasse derivative $t$. The polynomials $f_{b,t}$ for $b\in S$ and $t\in \Z_{\ge 0},\text{wt}(t)<l$ form a basis of $\F^{|S|L}$ via $\phi$. This proves $\text{Alg}^{(l)}(S)$ is isomorphic to $\F^{|S|L}$ as a vector space via $\phi$ and hence is $|S|L$ dimensional.

% We look at another interpretation for the evaluation map which well help us prove the second statement. The evaluation map can be interpreted as the isomorphism induced between $\text{Alg}(S,l)$ and the ring $\bigoplus_{b\in S}\F[X]/\langle X-b\rangle^l$ via canonical quotient maps $\F[X]\rightarrow \F[X]/\langle X-b\rangle^l$ where $X=(x_1,\hdots,x_n)$ and $\langle X-b\rangle=\langle x_1-b_1,\hdots,x_n-b_n\rangle$. The only thing which remains to be checked to verify this statement is whether the map is a ring homomorphism which is easy.

To prove the second statement, we will bound the dimension of $\text{Alg}^(l)(S)/\I_\F(W)$ where $W$ is a $k$-dimensional $(S,m)$-rich subspace. $\I_\F(W)$ is generated by $n-k$ linearly independent hyperplanes containing $W$. Because $\bigoplus_{b\in S}\F[X]/\langle X-b\rangle^l$ is isomorphic to $\text{Alg}^(l)(S)$ via the map $\phi$, to bound the dimension of $\text{Alg}(S,l)/\I_\F(W)$ we can simply examine $\left(\F[X]/\langle X-b\rangle^l\right)/\I_\F(W)$. If $W$ doesn't contain $b$ then some hyperplane $h$ containing $W$ will not contain $b$. That is $h\not\in \langle X-b\rangle$. This means $h$ is a unit in $\F[X]/\langle X-b\rangle^l$ because $\langle X-b\rangle$ is its only maximal ideal and $h$ is not in it. In this case $\left(\F[X]/\langle X-b\rangle^l\right)/\I_\F(W)=0$. If $\I_\F(W)$ contains $b$ we can perform a translation operation such that $b=0$. This means that we just need to examine $ \left(\F[X]/\langle X\rangle^l\right)/\I_\F(W)$ where $W$ is a $k$-dimensional subspace containing the origin. $\I_\F(W)$ will be generated by $n-k$ hyperplanes passing through the origin. We can perform a change of basis in $\F^n$ to ensure these hyperplanes are $x_1,\hdots,x_{n-k}$. This shows that $\left(\F[X]/\langle X\rangle^l\right)/\I_\F(W)$ is a ${l+k-1 \choose k}$ dimesnional vector space. This proves $\text{Alg}^{(l)}(S)/\I_\F(W)$ is of dimension at least $m{l+k-1 \choose k}$ if $W$ is $(S,m)$-rich.
\end{proof}
\begin{cor}\label{cor:MultAlgeb}
Given a $(k,m)$-Furstenberg set $S\subseteq \F^n$, for all $l\ge 1$ $\text{Alg}^{(l)}(S)$ is a finite dimensional algebra of dimension $|S|{l-1+n\choose n}$ which is $\left(k,m{l-1+k\choose k}\right)$-Furstenberg.
\end{cor}


\section{Proof of Theorem \ref{parametricBound}}\label{sec:ProofParameteric}

We are now ready to prove Theorem \ref{parametricBound}. As mentioned earlier the argument would produce a Hom-Furstenberg Algebra from Furstenberg set by using Corollary \ref{cor:MultAlgeb}. We then will recursively apply Theorem \ref{sec:nuancedBound} to obtain the desired bound. We restate the Theorem for convenience.


\begin{repthm}{parametricBound}
Given a $(k,m)$-Furstenberg Set $S\subseteq \F_q^n$ with $m=q^{(1-\epsilon)k},\epsilon\in (0,0.5]$ and 
$$q\ge (2e^3n^2)^{1/\epsilon},$$ 
we have the following bound,
$$|S|\ge  \left(\frac{1}{2e}\right)^{n-k+1}m^{n/k}.$$
\end{repthm}
% Note, we can prove other versions of this theorem where if $q$ is larger we get better constants in the theorem above.
\begin{proof}
We will use some standard inequalities,
\begin{align} 
\sum\limits_{i=r}^t \frac{1}{i}&\le \ln\left(
\frac{t}{r-1}\right) \label{eq:HarmonicBound}, \\
\sum\limits_{i=r}^t \frac{1}{i}&\ge \ln\left(
\frac{t}{r-1}\right)+\frac{1-t}{t} \label{eq:HarmonicUpperBound},\\
\ln(x+1)&\le x, \label{eq:LogarBound}\\
(1+x)^{1/n}&\le 1+\frac{x}{n}.\label{eq:powerBound}
\end{align}

Given a $(k,m)$-Furstenberg set $S$, $R=\text{hd}(\text{Alg}^{(n+1)}(S))$ is a $|S|{2n\choose n}$ dimensional algebra which is $(k,m{n+k\choose k})$-Hom-Furstenberg using Corollary \ref{cor:MultAlgeb} and Lemma \ref{DFrustLem}. Let $m_k=m{n+k\choose k}$. 
% We will take,
% \begin{align}
%  q\ge k^2(e^3n(\frac{n}{k}+1))^{1/\epsilon}\ge k^{2}(\Omega(\frac{n^2}{k}))^{1/\epsilon}.   \label{Qboundk}
% \end{align}

% Let $F_i=e^{-\sum_{r=k+2}^i 1/r}$ for $i>k+1$ and $F_{k+1}=1$. Using Equation \eqref{eq:HarmonicBound}, we have 
% \begin{align}
%     F_i \le e(k+1)/(i+1). \label{eq:Fibound}
% \end{align}

We will prove $R$ is $(j,m_j)$-Furstenberg with the bound
\begin{align}
    m_j\ge m_k^{j/k}\Bigg/\left(\prod\limits_{i=k+1}^{j} \left(e+\frac{1}{eni} \right)^{j/i}\right). \label{InducFr}
\end{align}
We will prove this recursively by going from dimension $j$ to $j+1$ as we did in the proof of Lemma \ref{recurseBound}.
We first examine the natural logarithm of the term $D_{n,j}=\prod_{i=k+1}^{j} \left(e+1/(eni) \right)^{j/i} $ in \eqref{InducFr}.
\begin{align*}
    \ln(D_{n,j})&=\sum\limits_{i=k+1}^j \frac{j}{i}\ln\left(e+\frac{1}{eni}\right) \\
    % \sum\limits_{i=k+1}^{j} \frac{j}{i}\ln\left(e+\frac{F_ii}{e^2nk(i-1)}\right)\\
    % &\le \sum\limits_{i=k+1}^j \frac{j}{i}\ln\left(e+\frac{i(k+1)}{enk(i^2-1)}\right) && \text{(Using \eqref{eq:Fibound})}\\
    % &\le \sum\limits_{i=k+1}^j \frac{j}{i}\ln\left(e+\frac{1}{n(i+1)}\right) && \text{(As }ik+i\le eki-ek\text{)}\\
    &\le \sum\limits_{i=k+1}^j \left(\frac{j}{i}+\frac{j}{e^2ni^2}\right)&& \text{ (Using \eqref{eq:LogarBound})}\\
    &\le j\ln\left(\frac{j}{k}\right)+\sum\limits_{i=k+1}^j \left(\frac{j}{eni}-\frac{j}{en(i+1)}\right) && \left(\text{ Using \eqref{eq:HarmonicBound} and }\frac{1}{ei^2}\le \frac{1}{i}-\frac{1}{i+1} \right)\\
    &\le j\ln\left(\frac{j}{k}\right)-\frac{j}{en(j+1)}+\frac{j}{en(k+1)} && \text{ (By telescoping)}\\
    \ln(D_{n,j})&\le j\ln\left(\frac{j}{k}\right)+\frac{j(j-k)}{en(j+1)(k+1)}\le j\ln\left(\frac{j}{k}\right)+\frac{j-k}{en(k+1)}. \label{DenomBound}\numberthis 
\end{align*}
Using \eqref{DenomBound} and the fact that $\epsilon\le 0.5$ shows,
\begin{align*}
% \Bigg(\frac{m_k^{j/k}}{\prod\limits_{i=k+1}^{j} \Big(e+e^{-1}F_ii/(i-1) \Big)^{j/i} }\Bigg)^{1/j}
m_k^{j/k}/D_{n,j} &\ge m^{j/k}{n+k \choose k}^{j/k}e^{-j\ln(\frac{j}{k})-\frac{j-k}{en(k+1)}}&& \text{(Using \eqref{DenomBound})}\\
&\ge m^{j/k}\frac{n^j}{k^j}\frac{k^j}{j^j}e^{-\frac{j-k}{en(k+1)}} && \left(\text{As }{n+k\choose k}\ge \frac{n^k}{k^k}\right)\\
&\ge m^{j/k}e^{-1/e} && \text{(As }n\ge j\ge j-k\text{)}\\
% &\ge q^{j(1-\epsilon)}e^{-1/e} && \text{(As }m=q^{k(1-\epsilon)}\text{)}\\
&\ge (2e^3n^2)^{j/\epsilon-j}e^{-1/e} &&\text{(As }m=q^{k(1-\epsilon)}\text{ and }q\ge (2e^{3}n^2)^{1/\epsilon}\text{)}\\
m_k^{j/k}/D_{n,j}&\ge (en)^{2j}\ge (ej)^{j}. \label{eq:FurstDnmBound} && \text{(As }\epsilon\le 0.5\text{)} \numberthis
\end{align*}



    
Now we prove \eqref{InducFr} by induction. For $j=k$, $S$ is $(k,m_k)$-Furstenberg. Equation \ref{eq:FurstDnmBound} implies $m_k\ge (ek)^{k}$ which means we can apply Theorem \ref{explicitHomFrust} for $S$. For $j=k+1$, note \begin{align}
    q^{-1}m_k^{1/k}\le q^{-\epsilon}{n+k\choose k}^{1/k}\le \frac{1}{2e^3n^2}e\frac{n+k}{k} \le \frac{1}{e^2nk}.
    \label{eq:baseqbound}
\end{align} This gives,
\begin{align*}
    m_{k+1}&\ge \frac{m_k^{(k+1)/k}}{e(1+(e^3nk)^{-1})^{1/k}+(e^2nk)^{-1}}\\
    &\ge \frac{m_k^{(k+1)/k}}{e+(e^2nk)^{-1}(k+1)/k} &&\text{ (Using Equation \eqref{eq:powerBound})}\\
    &\ge \frac{m_k^{(k+1)/k}}{e+(enk)^{-1}}.
\end{align*}
This proves \eqref{InducFr} for $j=k+1$. Let the statement be true for $j$. Again \eqref{eq:FurstDnmBound} shows $m_j\ge (ej)^{j}$, this means we can apply Theorem \ref{explicitHomFrust}. As in the proof of Lemma \ref{recurseBound} for any $j+1$ dimensional linear subspace $W$, $R/\langle \I_\F(W)\rangle$ will be $(j,m_j)$-Hom-Furstenberg Algebra in an appropriate set of $j+1$ coordinates. Applying Theorem \ref{explicitHomFrust} shows that $R$ is $(j+1,m_{j+1})$-Hom-Furstenberg with the bound,
\begin{align*}
    m_{j+1}&\ge \frac{m_j^{(j+1)/j}}{(e(1+e^{-1}q^{-1}m_j^{1/j})^{1/j}+q^{-1}m_j^{1/j})}\\
    &\ge \frac{m_j^{(j+1)/j}}{(e+q^{-1}m_j^{1/j}(j+1)/j)}.&&\text{ (Using Equation \eqref{eq:powerBound})}\numberthis \label{eq:nearFinbound}
\end{align*}
% \eqref{Qboundk}
The induction hypothesis and the fact that $q\ge (2e^3n^2)^{1/\epsilon}$ implies 
\begin{align*}
q^{-1}m_j^{1/j}&\le q^{-1}m_k^{1/k}e^{-\sum_{r=k+2}^j 1/r} && \text{(Using the induction hypothesis)}\\
% &=q^{-\epsilon}m_k^{}F_j && \left(\text{As }{n +k \choose k}\le \left(\frac{e(n+k)}{k}\right)^k\right) \\
% &=q^{-\epsilon}e(n+k)\frac{F_j}{k} && \left(\text{As }{n +k \choose k}\le \left(\frac{e(n+k)}{k}\right)^k\right) \\
&\le \frac{1}{en(j+1)}. && (\text{Using  \eqref{eq:HarmonicUpperBound} and \eqref{eq:baseqbound}})
\end{align*}
Applying the previous equation with equation \eqref{eq:nearFinbound} and the induction hypothesis gives us,
\begin{align*}
    m_{j+1}&\ge \frac{m_k^{(j+1)/k}}{D_{n,j}^{(j+1)/j} }\frac{1}{(e+q^{-1}m_j^{1/j}(j+1)/j)}\ge\frac{m_k^{(j+1)/k}}{D_{n,j}^{(j+1)/j}}\frac{1}{(e+1/(enj))}\ge \frac{m_k^{(j+1)/k}}{D_{n,j+1}} .
\end{align*}
Proving \eqref{InducFr} for all $j$. As $m_n=|R|=|S|{2n \choose n}$ using \eqref{InducFr} we have,
\begin{align*}
    |S|&\ge {2n \choose n}^{-1}\frac{m_k^{n/k}}{\prod\limits_{i=k+1}^{n} \Big(e+(e^2kn)^{-1}F_ii/(i-1) \Big)^{n/i}}\\
    &\ge {2n \choose n}^{-1}{n+k\choose k}^{n/k}e^{-n\ln(\frac{n}{k})-\frac{n-k}{en(k+1)}}m^{n/k}&& \text{(Using \eqref{DenomBound})}\\
    &\ge \frac{n!(n+k)!}{k!(2n)!}{n+k\choose k}^{(n-k)/k}\frac{k^n}{n^n}e^{-\frac{n-k}{en(k+1)}}m^{n/k}\\
    &\ge \frac{(n+k)^{n-k}}{(2n)^{n-k}} \frac{n!}{k!}\frac{k^n}{n^n}e^{-\frac{n-k}{en(k+1)}} m^{n/k} && \left(\text{Using }{n+k\choose k}\ge \frac{(n+k)^k}{k^k}\right)\\
    &\ge \left(1+\frac{k}{n}\right)^{n-k}\frac{1}{2^{n-k}} \frac{1}{e^{n-k+1}}e^{-\frac{n-k}{en(k+1)}}m^{n/k} &&\left(\text{As }\frac{n!}{k!}\ge \frac{n^n}{k^ke^{n-k+1}}\right)\\
    &\ge \left(\frac{1}{2e}\right)^{n-k+1}m^{n/k}.&& \left(\text{As }e^{-\frac{n-k}{en(k+1)}}\ge \frac{1}{2}\right)
\end{align*}


\end{proof}



% \label{dilationLem}

% \section{Extending the bound further by throwing away points}

% \begin{lem}[Throwing away points]\label{ThrowAwayLemma}
% Given a $(k,m)$-Furstenberg Set $S\subseteq \F^n_q$ and a $t,p\in [0,1]$ satisfying the bound,
% $$(q^{k(n-k)}{n \choose k}+1)e^{-2p^2m^3t^2}<1 $$
% we can find a subset $S'$ of $S$ with size at least $p|S|(1-t)$ such that it is $(k,mp(1-t))$-Furstenberg.
% \end{lem}
% \begin{proof}
% Consider the random process where we get a new set $S_p$ after randomly throwing away points independently with probability $1-p$. Using Hoeffding's inequality we have,
% $$ P(|S_p|\le p|S|(1-t))\le e^{-2p^2|S|^3t^2}.$$
% % where at the last step we used the fact $D(n,m)\le 1$.
% Given any $(S,m)$-rich $k$-dimensional subspace $V$ using Hoeffding's inequality we have,
% $$ P(|V\cap S_p|\le pm(1-t))\le e^{-2p^2m^3t^2}.$$
% Let the number of $k$-dimensinal linear subspaces be $G$. Applying union bound we note if
% $$e^{-2p^2|S|^3t^2}+Ge^{-2p^2m^3t^2}<1, $$
% then there exists a subset $S'$ of $S$ with size at least $p|S|(1-t)$ which is $(k,mp(1-t))$-Furstenberg. $|G|\le q^{k(n-k)}{n \choose k}$ and $|S|<m$ we can use the sufficient condition,
% $$(q^{k(n-k)}{n \choose k}+1)e^{-2p^2m^3t^2}<1.$$
% \end{proof}

% We want to use Lemma \ref{ThrowAwayLemma} to extend the bound obtained in the previous section.

% \begin{thm}[Products of Furstenberg Sets]\label{productSets}
% Given a $(k_1, m_1)$-Furstenberg set $S\subseteq \F^n$ and a $(k_2,m_2)$-Furstenberg set $T\subseteq \F^n$, $S\times T\subseteq \F^{2n}$ is a $(k_1+k_2,m_1m_2)$-Furstenberg set.
% \end{thm}
% \begin{proof}
% A $k_1+k_2$ dimensional vector space
% \end{proof}








% \begin{lem}[Borel fixed lattice bound]\label{latticeBound}
% Given a Borel fixed lattice $\Lambda$, let $\Lambda_n$ be the subset of $\Lambda$ lying on the plane $\lambda_n=0$. If $|\Lambda_n|\ge m$ then 
% $$|\Lambda|\ge \frac{1}{D}m^{n/(n-1)},$$
% where $D$ is some universal constant.
% \end{lem}
% \begin{proof}
% We have $|\Lambda_n|\ge m$. We first discuss the case of $n=2$ which gives a simplified picture of the full argument. First, we throw away points in $\Lambda_2$ for which $\lambda_1<m/2$. We still would have at least $m/2$ points left in $\Lambda_2$. Given any point $\lambda=(\lambda_1,0)\in \Lambda_0$ we produce lattice points $(l,\lambda_2-l)\in \Lambda$ for $0\le l \le \lambda_2$. We collect these points in a set $\PATH(\lambda)$. The points in $\PATH(\lambda)$ are the non-negative lattice points on the line along the direction $\ce_1-\ce_2$ starting from the point $\lambda$. This implies, for two distinct points $\lambda$ and $\mu$ in $\Lambda_2$, $\PATH(\lambda)$ and $\PATH(\mu)$ will be disjoint. For each point $\lambda$, $|\PATH(\lambda)|$ will be at least of size $m/2$. This gives us the lower bound $|\Lambda|\ge m^2/4$. 

% From now on we take $n\ge 3$. We let ${r \choose a}=\frac{r(r-1)(r-2)\hdots(r-a+1)}{a!}$ where $r$ is a real number and $a$ a non-negative integer. We can find a positive real number $d$ such that, 
% $$m={n-1 + d \choose n-1}.$$ 
% We will assume $m\ge (2e)^{n-1}$. This is fine as long as $D\ge 2e$. Using this assumption we have the bound 
% \begin{align*}
% &(2e)^{n-1}\le m={n-1 + d \choose n-1}\le \frac{(n-1+d)^{n-1}}{(n-1)!}\\
% \implies & 2e((n-1)!)^{1/(n-1)}\le n-1+d\\
% \implies & n-1\le d.
% \end{align*}
% For the last step we used the bound $n^n\le e^nn!$. For a lattice point $\lambda$, we recall $\text{wt}(\lambda)=\sum_i \lambda_i$. The number of lattice points with weight less than $d/2$ are at most ${n-1+d/2 \choose n-1}$. If we throw out these points from $\Lambda_n$ we still have at least 
% \begin{align*}
%      m(1-\frac{n-1+d/2}{n-1+d}\hdots\frac{2+d/2}{2+d}\frac{1+d/2}{1+d}) &\ge m(1-\frac{2+d/2}{2+d}\frac{1+d/2}{1+d})  \\
%      &\ge m(1-\frac{1}{2}\frac{2+d/2}{1+d}) \\
%     &\ge m/2
% \end{align*} 
% points in $\Lambda_n$ where at the last step we used $d\ge n-1$ and $n\ge 3$.

% For any point $\lambda=(\lambda_1,\hdots,\lambda_{n-1},0)\in \Lambda_n$ we will produce points in $\Lambda$ as before. This time we will construct $\PATH(\lambda)$ in $n-1$ stages. In stage $1$, we start at $\lambda=P_1(\lambda)$ and we move along the direction $\ce_n-\ce_{n-1}$ until we hit the hyperplane $\lambda_{n-1}=0$ producing the lattice points $(\lambda_1,\lambda_2,\hdots,\lambda_{n-1}-l,l)\in \Lambda$ for all $0< l\le \lambda_{n-1}$, as $\Lambda$ is Borel fixed. We collect these points in the set $\PATH(\lambda,1)$. We note $|\PATH(\lambda,1)|=\lambda_{n-1}$. At the end of stage $1$ we are at the point $P_2(\lambda)=(\lambda_1,\hdots,\lambda_{n-2},0,\lambda_{n-1})\in \Lambda$. 

% In general, at stage $i$ we start at the point $P_i(\lambda)=(\lambda_1,\hdots,\lambda_{n-i},0,\lambda_{n-i+1},\hdots,\lambda_{n-1})$. We then move along the direction $\ce_{n-i+1}-\ce_{n-i}$ until we hit the hyperplane $\lambda_{i+1}=0$ producing lattice points $(\lambda_1,\hdots,\lambda_{n-i}-l,l,\lambda_{n-i+1},\hdots,\lambda_{n-1})\in \Lambda$ for $0<l\le \lambda_{n-i}$. We collect these points in $\PATH(\lambda,i)$ which has size $\lambda_{n-i}$. At the end of stage $i$ we are at the point $P_{i+1}(\lambda)=(\lambda_1,\hdots,\lambda_{n-i-1},0,\lambda_{n-i},\hdots,\lambda_{n-1})$. There are $n-1$ stages. We set $\PATH(\lambda)=\bigcup_{i=1}^{n-1}\PATH(\lambda,i)$. We note, $|\PATH(\lambda)|=\sum_{i=1}^{n-1} |\PATH(\lambda,i)|=\sum_{i=1}^{n-1} \lambda_i\ge d/2$. Unlike the case of $n=2$, for distinct points $\lambda$ and $\mu$ in $\Lambda_n$, $\PATH(\lambda)$ and $\PATH(\mu)$ may not be disjoint. We are going to bound the number of times this can happen.

% Say $\alpha\in \bigcup_{\lambda \in \Lambda_n}\PATH(\lambda)$. We claim for all $1\le i\le n-1$, there exists at most one point $\lambda \in \Lambda_n$ such that $\alpha \in \PATH(\lambda,i)$. Say there exists two such points $\lambda=(\lambda_1,\hdots,\lambda_{n-1},0)$ and $\mu=(\mu_1,\hdots,\mu_{n-1},0)$. Let $\alpha=(\alpha_1,\hdots,\alpha_n)$. As $\lambda$ and $\mu$ produced $\alpha$ in stage $i$, there exists $l_1$ and $l_2$ such that
% \begin{align*}
%     \alpha &= (\alpha_1,\hdots,\alpha_{n-i},\alpha_{n-i+1},\alpha_{n-i+2}\hdots,\alpha_{n})\\
%     &= (\lambda_1,\hdots,\lambda_{n-i}-l_1,l_1,\lambda_{n-i+1},\hdots,\lambda_{n-1}) \\
%     &= (\mu_1,\hdots,\mu_{n-i}-l_2,l_2,\mu_{n-i+1},\hdots,\mu_{n-1}).
% \end{align*}
% This implies $\lambda_j=\mu_j=\alpha_j$ for $1\le j\le n-i-1$, $\lambda_{j}=\mu_j=\alpha_{j+1}$ for $n-i+1\le j\le n-1$, and $\lambda_{n-i}=\mu_{n-i}=\alpha_{n-i}+\alpha_{n-i+1}$. This proves $\lambda=\mu$. This claim then implies there are at most $n-1$ points $\lambda$ in $\Lambda_n$ such that $\alpha \in \PATH(\lambda)$. 

% Each $\PATH(\lambda)$ is of size at least $d/2$. Combining this with the fact proven in the previous paragraph gives us a lower bound for the size of $\Lambda$,
% $$|\Lambda|\ge \frac{d}{2(n-1)}\frac{m}{2}=\frac{1}{4}\frac{d}{n-1}{n-1 + d \choose n-1}.$$
% We note,
% $${n-1 + d \choose n-1}^{-1/(n-1)}\frac{d}{n-1}=\frac{((n-1)!)^{1/(n-1)}}{n-1}\Big(\frac{d}{n-1+d}\hdots\frac{d}{1+d}\Big)^{1/(n-1)}\ge \frac{1}{2e}$$
% where at the last step we used the fact that $d\ge n-1$ and $n^n\le e^nn!$. Using this we get the required bound,
% $$|\Lambda|\ge \frac{1}{8e}m^{n/(n-1)}. $$
% \end{proof}
